Entanglement-Assisted Bosonic MAC: Achievable Rates and Covert Communication

We consider the problem of covert communication over the entanglement-assisted (EA) bosonic multiple access channel (MAC). We derive a closed-form achievable rate region for the general EA bosonic MAC using high-order phase-shift keying (PSK) modulation. Specifically, we demonstrate that in the low-photon regime the capacity region collapses into a rectangle, asymptotically matching the point-to-point capacity as multi-user interference vanishes. We also characterize an achievable covert throughput region, showing that entanglement assistance enables an aggregate throughput scaling of \(O(\sqrt{n} \log n)\) covert bits with the block length $n$ for both senders, surpassing the square-root law as in the point-to-point case. Our analysis reveals that the joint covertness constraint imposes a linear trade-off between the senders throughput.

==> Acronyms.tex <==
\acrodef{ACDIS}[ACDIS]{Adaptive Communication Decision and Information Systems}
\acrodef{AEP}{Asymptotic Equipartition Property}
\acrodef{AoA}{Angle of Arrival}
\acrodef{AWGN}{Additive White Gaussian Noise}
\acrodef{AVC}[AVC]{Arbitrarily Varying Channel}
\acrodef{BER}{Bit-Error-Rate}
\acrodef{BEC}{Binary Erasure Channel}
\acrodef{BPSK}{Binary Phase-Shift Keying}
\acrodef{BSC}{Binary Symmetric Channel}
\acrodef{BICM}[BICM]{Bit-Interleaved Coded-Modulation}
\acrodef{CDF}[CDF]{Cumulative Distribution Function}
\acrodef{CGF}[CGF]{Cumulant Generating Function}
\acrodef{CLT}[CLT]{Central Limit Theorem}
\acrodef{cq}[c-q]{Classical-Quantum}
\acrodef{CSI}[CSI]{Channel State Information}
\acrodef{DMC}[DMC]{Discrete Memoryless Channel}
\acrodef{DMS}[DMS]{Discrete Memoryless Source}
\acrodef{ERM}[ERM]{Empirical Risk Minimization}
\acrodef{FER}[FER]{Frame Error Rate}
\acrodef{ICA}[ICA]{Independent Component Analysis}
\acrodef{iid}[i.i.d.]{independent and identically distributed}
\acrodef{IoT}[IoT]{Internet of Things}
\acrodef{KKT}[KKT]{Karush-Kuhn Tucker}
\acrodef{LASSO}[LASSO]{Least Absolute Shrinkage and Selection Operator}
\acrodef{LPD}[LPD]{Low Probability of Detection}
\acrodef{LDPC}[LDPC]{Low-Density Parity-Check}
\acrodef{LLMS}[LLMS]{Linear Least Mean Square}
\acrodef{LMS}[LMS]{Least Mean Square}
\acrodef{MAC}[MAC]{multiple-access channel}
\acrodef{MGF}[MGF]{Moment Generating Function}
\acrodef{MLC}[MLC]{Multi-Level Coding}
\acrodef{MLE}[MLE]{Maximum Likelihood Estimate}
\acrodef{MIMO}[MIMO]{Multiple-Input Multiple-Output}
\acrodef{MISO}{Multiple-Input Single-Output}
\acrodef{MSD}[MSD]{Multi-Stage Decoding}
\acrodef{MMSE}[MMSE]{Minimum Mean-Square Error}
\acrodef{PAC}[PAC]{Probably Approximately Correct}
\acrodef{PCA}[PCA]{Principal Component Analysis}
\acrodef{PDF}[PDF]{Probability Density Function}
\acrodef{PMF}[PMF]{Probability Mass Function}
\acrodef{POVM}[POVM]{Positive Operator-Valued Measure}
\acrodef{PVM}[PVM]{Projection-Valued Measure}
\acrodef{PPM}[PPM]{Pulse Position Modulation}
\acrodef{PSD}{Power Spectral Density}
\acrodef{PSK}{Phase Shift Keying}
\acrodef{QKD}{Quantum Key Distribution}
\acrodef{ROC}{Receiver Operating Characteristic}
\acrodef{CVQKD}{Continuous-Variable \ac{QKD}}
\acrodef{QPSK}{Quadrature Phase-Shift Keying}
\acrodef{RV}{random variable}
\acrodef{SIMO}{Single-Input Multiple-Output}
\acrodef{SNR}{Signal-to-Noise Ratio}
\acrodef{SVM}[SVM]{Support Vector Machine}
\acrodef{TPCP}{Trace-Preserving Completely-Positive}
\acrodef{wrt}[w.r.t.]{with respect to}
\acrodef{WSS}{Wide Sense Stationary}


==> CommandsAndMacros.tex <==
\newcommand{\matA}{\mathbf{A}}
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\veca}{\mathbf{a}}
\newcommand{\matB}{\mathbf{B}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\matC}{\mathbf{C}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\vecc}{\mathbf{c}}
\newcommand{\matD}{\mathbf{D}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\vecd}{\mathbf{d}}
\newcommand{\matE}{\mathbf{E}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\matF}{\mathbf{F}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\vecf}{\mathbf{f}}
\newcommand{\matG}{\mathbf{G}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\matH}{\mathbf{H}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\vech}{\mathbf{h}}
\newcommand{\matI}{\mathbf{I}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\veci}{\mathbf{i}}
\newcommand{\matJ}{\mathbf{J}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\vecj}{\mathbf{j}}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\veck}{\mathbf{k}}
\newcommand{\matL}{\mathbf{L}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\vecl}{\mathbf{l}}
\newcommand{\matM}{\mathbf{M}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\vecm}{\mathbf{m}}
\newcommand{\matN}{\mathbf{N}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\matO}{\mathbf{O}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\veco}{\mathbf{o}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\vecp}{\mathbf{p}}
\newcommand{\matQ}{\mathbf{Q}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\vecq}{\mathbf{q}}
\newcommand{\matR}{\mathbf{R}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\matS}{\mathbf{S}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\vecs}{\mathbf{s}}
\newcommand{\matT}{\mathbf{T}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\vect}{\mathbf{t}}
\newcommand{\matU}{\mathbf{U}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\vecu}{\mathbf{u}}
\newcommand{\matV}{\mathbf{V}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\matW}{\mathbf{W}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\matY}{\mathbf{Y}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\matZ}{\mathbf{Z}}
\newcommand{\bfZ}{\mathbf{Z}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bfz}{\mathbf{z}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\bfalpha}{\boldsymbol{\alpha}}
\newcommand{\vecalpha}{\boldsymbol{\alpha}}
\newcommand{\bfbeta}{\boldsymbol{\beta}}
\newcommand{\vecbeta}{\boldsymbol{\beta}}
\newcommand{\bfgamma}{\boldsymbol{\gamma}}
\newcommand{\vecgamma}{\boldsymbol{\gamma}}
\newcommand{\bfdelta}{\boldsymbol{\delta}}
\newcommand{\vecdelta}{\boldsymbol{\delta}}
\newcommand{\bfepsilon}{\boldsymbol{\epsilon}}
\newcommand{\vecepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bfzeta}{\boldsymbol{\zeta}}
\newcommand{\veczeta}{\boldsymbol{\zeta}}
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\veceta}{\boldsymbol{\eta}}
\newcommand{\bftheta}{\boldsymbol{\theta}}
\newcommand{\vectheta}{\boldsymbol{\theta}}
\newcommand{\bfiota}{\boldsymbol{\iota}}
\newcommand{\veciota}{\boldsymbol{\iota}}
\newcommand{\bfkappa}{\boldsymbol{\kappa}}
\newcommand{\veckappa}{\boldsymbol{\kappa}}
\newcommand{\bflamda}{\boldsymbol{\lamda}}
\newcommand{\veclamda}{\boldsymbol{\lamda}}
\newcommand{\bfmu}{\boldsymbol{\mu}}
\newcommand{\vecmu}{\boldsymbol{\mu}}
\newcommand{\bfnu}{\boldsymbol{\nu}}
\newcommand{\vecnu}{\boldsymbol{\nu}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\vecxi}{\boldsymbol{\xi}}
\newcommand{\bfomicron}{\boldsymbol{\omicron}}
\newcommand{\vecomicron}{\boldsymbol{\omicron}}
\newcommand{\bfpi}{\boldsymbol{\pi}}
\newcommand{\vecpi}{\boldsymbol{\pi}}
\newcommand{\bfrho}{\boldsymbol{\rho}}
\newcommand{\vecrho}{\boldsymbol{\rho}}
\newcommand{\bfsigma}{\boldsymbol{\sigma}}
\newcommand{\vecsigma}{\boldsymbol{\sigma}}
\newcommand{\bftau}{\boldsymbol{\tau}}
\newcommand{\vectau}{\boldsymbol{\tau}}
\newcommand{\bfupsilon}{\boldsymbol{\upsilon}}
\newcommand{\vecupsilon}{\boldsymbol{\upsilon}}
\newcommand{\bfphi}{\boldsymbol{\phi}}
\newcommand{\vecphi}{\boldsymbol{\phi}}
\newcommand{\bfchi}{\boldsymbol{\chi}}
\newcommand{\vecchi}{\boldsymbol{\chi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\vecpsi}{\boldsymbol{\psi}}
\newcommand{\bfomega}{\boldsymbol{\omega}}
\newcommand{\vecomega}{\boldsymbol{\omega}}
\newcommand{\bfAlpha}{\boldsymbol{\Alpha}}
\newcommand{\matAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bfBeta}{\boldsymbol{\Beta}}
\newcommand{\matBeta}{\boldsymbol{\Beta}}
\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\matGamma}{\boldsymbol{\Gamma}}
\newcommand{\bfDelta}{\boldsymbol{\Delta}}
\newcommand{\matDelta}{\boldsymbol{\Delta}}
\newcommand{\bfEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\matEpsilon}{\boldsymbol{\Epsilon}}
\newcommand{\bfZeta}{\boldsymbol{\Zeta}}
\newcommand{\matZeta}{\boldsymbol{\Zeta}}
\newcommand{\bfEta}{\boldsymbol{\Eta}}
\newcommand{\matEta}{\boldsymbol{\Eta}}
\newcommand{\bfTheta}{\boldsymbol{\Theta}}
\newcommand{\matTheta}{\boldsymbol{\Theta}}
\newcommand{\bfIota}{\boldsymbol{\Iota}}
\newcommand{\matIota}{\boldsymbol{\Iota}}
\newcommand{\bfKappa}{\boldsymbol{\Kappa}}
\newcommand{\matKappa}{\boldsymbol{\Kappa}}
\newcommand{\bfLamda}{\boldsymbol{\Lamda}}
\newcommand{\matLamda}{\boldsymbol{\Lamda}}
\newcommand{\bfMu}{\boldsymbol{\Mu}}
\newcommand{\matMu}{\boldsymbol{\Mu}}
\newcommand{\bfNu}{\boldsymbol{\Nu}}
\newcommand{\matNu}{\boldsymbol{\Nu}}
\newcommand{\bfXi}{\boldsymbol{\Xi}}
\newcommand{\matXi}{\boldsymbol{\Xi}}
\newcommand{\bfOmicron}{\boldsymbol{\Omicron}}
\newcommand{\matOmicron}{\boldsymbol{\Omicron}}
\newcommand{\bfPi}{\boldsymbol{\Pi}}
\newcommand{\matPi}{\boldsymbol{\Pi}}
\newcommand{\bfRho}{\boldsymbol{\Rho}}
\newcommand{\matRho}{\boldsymbol{\Rho}}
\newcommand{\bfSigma}{\boldsymbol{\Sigma}}
\newcommand{\matSigma}{\boldsymbol{\Sigma}}
\newcommand{\bfTau}{\boldsymbol{\Tau}}
\newcommand{\matTau}{\boldsymbol{\Tau}}
\newcommand{\bfUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\matUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bfPhi}{\boldsymbol{\Phi}}
\newcommand{\matPhi}{\boldsymbol{\Phi}}
\newcommand{\bfChi}{\boldsymbol{\Chi}}
\newcommand{\matChi}{\boldsymbol{\Chi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\matPsi}{\boldsymbol{\Psi}}
\newcommand{\bfOmega}{\boldsymbol{\Omega}}
\newcommand{\matOmega}{\boldsymbol{\Omega}}
\newcommand{\bfzero}{\boldsymbol{0}}

\newcommand{\card}[1]{{|{#1}|}}
\newcommand{\abs}[1]{{\left|{#1}\right|}}
\newcommand{\sgn}[1]{{\text{sgn}\left({#1}\right)}}
\newcommand{\norm}[2][]{{\left\Vert{#2}\right\Vert}_{#1}}
\newcommand{\inprod}[3][]{{\left\langle{#2},{#3}\right\rangle}_{#1}}
\newcommand{\dotp}[3][]{{\left\langle{#2},{#3}\right\rangle}_{#1}}
\newcommand{\set}[1]{{\{#1\}}}
\newcommand{\trace}[1]{\text{trace}\left(#1\right)}
\newcommand{\argmin}{\mathop{\text{argmin}}}
\newcommand{\argmax}{\mathop{\text{argmax}}}
\newcommand{\intseq}[2]{[{#1};{#2}]}
\newcommand{\eqdef}{\triangleq}
\newcommand{\E}[2][]{{\mathbb{E}_{#1}\left[#2\right]}}
\newcommand{\Var}[1]{{\text{Var}\left(#1\right)}}
\newcommand{\Cov}[1]{{\text{Cov}\left(#1\right)}}
\renewcommand{\P}[2][]{{\mathbb{P}_{#1}\left(#2\right)}}
\newcommand{\indic}[1]{{\mathbf{1}\{#1\}}}
\newcommand{\mat}[2]{\left[\begin{array}{#1}#2\end{array}\right]}
\newcommand{\bra}[1]{{\left\langle{#1}\right\vert}}
\newcommand{\ket}[1]{{\left\vert{#1}\right\rangle}}

\newcommand{\D}[3][]{{\mathbb{D}_{#1}}\!\left(#2\,\middle\Vert\,#3\right)} % divergence
\newcommand{\V}[3][]{{\mathbb{V}_{#1}}\!\left(#2,#3\right)} % total variation
\newcommand{\I}[2]{{{\mathbb{I}}\!\left(#1;#2\right)}} % mutual information (two params)
\newcommand{\avgI}[1]{{{\mathbb{I}}\!\left(#1\right)}} % mutual information
\newcommand{\avgH}[1]{{\mathbb{H}}\!\left(#1\right)}
\newcommand{\h}[1]{{{h}}\left(#1\right)} % differential entropy
\newcommand{\Hb}[1]{{h_b}\left(#1\right)} % Binary entropy function

\newcommand{\GF}[1]{\ensuremath{\mbox{GF}(#1)}} % Galois field
\newcommand{\F}[1]{\ensuremath{\mathbb{F}_{#1}}} % Field
\newcommand{\dH}[1]{\ensuremath{\mbox{d}_{\mbox{\tiny H}}(#1)}} % Hamming distance
\newcommand{\wt}[1]{\ensuremath{\mbox{wt}(#1)}} % Weight of a vector

\newcommand{\dd}{\text{\textnormal{d}}} % differential operator as in dx
\renewcommand{\leq}{\leqslant} % redefines <=
\renewcommand{\geq}{\geqslant} % redefines >=


% Matrix operations
\newcommand{\tr}[2][]{\ensuremath{\text{\textnormal{tr}}_{#1}\left(#2\right)}}  % Trace
\newcommand{\rk}[1]{\ensuremath{\text{\textnormal{rank}}\left(#1\right)}}  % Rank
\renewcommand{\det}[1]{{\left|{#1}\right|}}                              % Det
\renewcommand{\ker}[1]{\ensuremath{\text{\textnormal{Ker}}\left(#1\right)}}  % Kernel
